Analyzing Machine Learning Workloads Using a Detailed GPU Simulator

Most deep neural networks deployed today are trained using GPUs via high-level frameworks such as TensorFlow and PyTorch. This paper describes changes we made to the GPGPU-Sim simulator to enable it to run PyTorch by running PTX kernels included in NVIDIA's cuDNN library. We use the resulting modified simulator, which has been made available publicly with this paper, to study some simple deep learning workloads. With our changes to GPGPU-Sim's functional simulation model, we find GPGPU-Sim performance model running a cuDNN enabled implementation of LeNet for MNIST reports results within 30% of real hardware. Using GPGPU-Sim's AerialVision performance analysis tool we observe that cuDNN API calls contain many varying phases and appear to include potentially inefficient microarchitecture behaviour such as DRAM partition bank camping, at least when executed on GPGPU-Sim's current performance model.

==> relatedWork.tex <==
\iffalse
\section{Related Tools}
\label{sec:relWork}



\subsection{NVProf}
\label{subsec:relWork-prof}

The most closely related tool to GPGPU-Sim is NVProf~\cite{nvprof}, NVIDIA's command-line profiler for CUDA programs.  NVProf and GPGPU-Sim give many similar statistics, including instructions per cycle and the number of instructions executed for certain types of instructions such as loads and stores. They also track basic memory and stall information. NVProf is useful in many cases since it provides fast, accurate results from the hardware itself. However, NVProf has many limitations concerning what statistics it can provide.  In comparison, GPGPU-Sim provides detailed information on memory usage, power, efficiency, and can output useful plots of relevant statistics using AerialVision.

Several recent papers have used tools like nvprof to profile ML 
workloads~\cite{SunMukherjee18-rocm, MojumderLouis18-volta, ZhuPhanishayee18-tbd}.  
Since these papers use profilers, unlike our work they can only provide higher-level analysis about the 
behaviors of the applications.

\subsection{Simulation}
\label{subsec:relWork-sim}

Some prior work has also simulated ML workloads, but these papers used private 
simulators~\cite{RhuOConnor18-cdma, ParasharRhu17-scnn, HanLiu2016-eie, AlbericioDelmas2017-bitprag}.  
Since these simulators are not publicly available and few details are available, it is difficult to precisely 
compare their approaches to ours.  In comparison, we simulate ML workloads at high fidelity in the widely used, 
publicly available GPGPU-Sim.  Moreover, the fact that other papers use disparate architectural simulators for ML 
workloads makes it crucial to provide public, widely used tools for simulating ML workloads.
\fi
